The Bias Amplification Paradox in Text-to-Image Generation

Bias amplification is a phenomenon in which models exacerbate biases or stereotypes present in the training data. In this paper, we study bias amplification in the text-to-image domain using Stable Diffusion by comparing gender ratios in training vs. generated images. We find that the model appears to amplify gender-occupation biases found in the training data (LAION) considerably. However, we discover that amplification can be largely attributed to discrepancies between training captions and model prompts. For example, an inherent difference is that captions from the training data often contain explicit gender information while our prompts do not, which leads to a distribution shift and consequently inflates bias measures. Once we account for distributional differences between texts used for training and generation when evaluating amplification, we observe that amplification decreases drastically. Our findings illustrate the challenges of comparing biases in models and their training data, and highlight confounding factors that impact analyses.

==> fig/circles.tex <==
\begin{tikzpicture}
  % Inner circle with divisions
  \draw (0,0) circle (3cm);
  \draw (0,0) -- (45:3cm); % 45 degrees
  \draw (0,0) -- (135:3cm); % 135 degrees
  \draw (0,0) -- (202.5:3cm); % 202.5 degrees
  \draw (0,0) -- (247.5:3cm); % 247.5 degrees
  
  % Labels
  \node at (22.5:3.4cm) {5\%};
  \node at (90:3.4cm) {45\%};
  \node at (168.75:3.4cm) {33\%};
  \node at (225:3.4cm) {17\%};
  
  % Outer circles (two half circles)
  \draw[red] (45:3cm) arc (45:135:6cm);
  \draw[blue] (135:3cm) arc (135:225:6cm);
\end{tikzpicture}

==> macros.tex <==
%\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{color}
\usepackage{times}
\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{bbm}
\usepackage{dsfont}


\usepackage[utf8]{inputenc}
\usepackage{booktabs,siunitx}
\usepackage{multirow}
\usepackage{multicol}
\usepackage{amsmath}
\usepackage{subcaption}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{pifont}


\usepackage{tikz}
\usetikzlibrary{shapes,arrows,patterns}
\usetikzlibrary{positioning}
% needed for BB
\usetikzlibrary{calc}


\newcommand{\loss}{\mathcal{L}}
\newtheorem{thm}{Theorem}
\newtheorem{lma}{Lemma}
% \usepackage[numbers]{natbib}

\newcommand{\relLabel}[1]{\texttt{#1}}

\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\newcommand{\cmark}{\textcolor{green!70!black}{\ding{51}}}%
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}%

\newtheorem{theorem}{Theorem}[section]
\newcommand{\sameer}[2][]{\textcolor{blue}{\textbf{sam:}\textbf{#1:} #2}}
\newcommand{\pouya}[1]{\textcolor{magenta}{\textbf{pouya:} #1}}
\newcommand{\preethi}[1]{\textcolor{green!50!black}{\textbf{preethi:} #1}}

% --------------------------------------------------------------
% --------------------------------------------------------------
% --------------------------------------------------------------
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\newcommand{\R}{\ensuremath{\mathcal{R}}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\meta}{\text{training-feature attribution}}
\newcommand{\metab}{\text{Training-Feature Attribution}}
\newcommand{\metas}{\text{TFA}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

\newcommand{\cut}[1]{}

\newcommand\tab[1][1cm]{\hspace*{#1}}
% \newcommand{\argmin}{\operatornamewithlimits{argmin}}

\newcommand{\imp}{\textcolor{red}{ERROR: \text{Mismatch}}}
\newcommand{\impu}{\text{Mismatch}}
%\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\postspace}{\vskip -3mm}
\newcommand{\minipostspace}{\vskip -2mm}
\newcommand{\prespace}{\vskip 1mm}
% \newcommand{\postspace}{}
% \newcommand{\minipostspace}{}

\newcommand{\tightcbox}[2]{\setlength{\fboxsep}{0pt}\colorbox{#1}{\strut #2}}
\definecolor{red}{RGB}{255, 117, 115}
\definecolor{green}{RGB}{171, 255, 175}



==> tables/BA_all_prompts.tex <==
\begin{table*}[t]
 \centering
 \small
  \begin{tabular}{llllll}
    \toprule        
    \bf Approach & \bf Model & \bf Prompt 1 & \bf Prompt 2 & \bf Prompt 3 & \bf Prompt 4 \\
    \midrule
    \multirow{ 2}{*}{Keyword Querying} & SD 1.4 & 10.24 & 17.57 & 10.77 & 11.68  \\
   &  SD 1.5 & 10.87 & 16.36 & 11.15 & 9.91 \\
   \midrule
   \multirow{ 2}{*}{Nearest Neighbors} & SD 1.4 & 3.59 & 12.62 & 5.58 & 5.27    \\
    & SD 1.5 & 4.01 & 11.14 & 5.21 & 3.65   \\
   \midrule
   \multirow{ 2}{*}{No Gender Indicators} & SD 1.4 & 6.49 & 13.58 & 7.09 & 7.49    \\
    & SD 1.5 & 6.76 & 12.41 & 6.82 & 5.87    \\
   \midrule
   % \multirow{ 2}{*}{
   Nearest Neighbors + & SD 1.4 & 1.11 & 8.72 & 3.06 & 4.05    \\
   No Gender Indicators & SD 1.5 & 1.55 & 7.29 &2.78 & 2.72   \\
    \bottomrule
  \end{tabular}
   \caption{Average Bias Amplification (BA) across occupations, for each prompt. Results are shown both for Stable Diffuson (SD) 1.4 and 1.5. For each prompt, bias amplification lowers considerably when using nearest neighbors to select training captions and excluding captions with gender indicators. We see further reductions when combining approaches.}
  \label{tab:results_prompts}
\end{table*}

==> tables/bias_amplification.tex <==
\begin{table}[t]
 \centering
 \small
  \begin{tabular}{lrr}
    \toprule        
    \bf Approach & \bf Model & \bf \thead{Bias\\Amplification} \\
    \midrule
    \multirow{ 2}{*}{Keyword Querying} & SD 1.4 & 12.57  \\
   &  SD 1.5 & 12.07  \\
   \midrule
   \multirow{ 2}{*}{Nearest Neighbors} & SD 1.4 & 6.76    \\
    & SD 1.5 & 6.01   \\
   \midrule
   \multirow{ 2}{*}{No Gender Indicators} & SD 1.4 & 8.66    \\
    & SD 1.5 & 7.97    \\
   \midrule
   % \multirow{ 2}{*}{
   Nearest Neighbors + & SD 1.4 & 4.35    \\
   No Gender Indicators & SD 1.5 & 3.59    \\
    \bottomrule
  \end{tabular}
   \caption{\textbf{Average bias amplification across occupations and prompts for both Stable Diffusion (SD) 1.4 and 1.5.} Amplification lowers when using nearest neighbors to select training captions and excluding captions with gender indicators, and further reduces when combining approaches.}
  \label{tab:results}
  \vspace{-1.0em}
\end{table}

==> tables/cos_sim.tex <==
\begin{table}[t]
 \centering
 \small
  \begin{tabular}{lll}
    \toprule        
    \bf Occupation & \bf \thead{Keyword\\ Querying} & \bf \textsc{NN} \\
    \midrule
    % Teacher & tr-tr & 0.416 & 0.699   \\
    Teacher & 0.469 & 0.570   \\
    % President & tr-tr & 0.446 & 0.561    \\
    President & 0.379 & 0.444    \\
     \addlinespace
     % All Occ & tr-tr & 0.472 & 0.639    \\
     All Occupations & 0.519 & 0.586    \\
    \bottomrule
  \end{tabular}
   \caption{Average pairwise cosine similarity between training and generated image embeddings. Embeddings are computed using CLIP's image encoder.}
   \vspace{-1.0em}
  \label{tab:emb}
\end{table}
